Better to Ask in English: Cross-Lingual Evaluation of Large Language Models for Healthcare Queries

Large language models (LLMs) are transforming the ways the general public accesses and consumes information. Their influence is particularly pronounced in pivotal sectors like healthcare, where lay individuals are increasingly appropriating LLMs as conversational agents for everyday queries. While LLMs demonstrate impressive language understanding and generation proficiencies, concerns regarding their safety remain paramount in these high-stake domains. Moreover, the development of LLMs is disproportionately focused on English. It remains unclear how these LLMs perform in the context of non-English languages, a gap that is critical for ensuring equity in the real-world use of these systems.This paper provides a framework to investigate the effectiveness of LLMs as multi-lingual dialogue systems for healthcare queries. Our empirically-derived framework XlingEval focuses on three fundamental criteria for evaluating LLM responses to naturalistic human-authored health-related questions: correctness, consistency, and verifiability. Through extensive experiments on four major global languages, including English, Spanish, Chinese, and Hindi, spanning three expert-annotated large health Q&A datasets, and through an amalgamation of algorithmic and human-evaluation strategies, we found a pronounced disparity in LLM responses across these languages, indicating a need for enhanced cross-lingual capabilities. We further propose XlingHealth, a cross-lingual benchmark for examining the multilingual capabilities of LLMs in the healthcare context. Our findings underscore the pressing need to bolster the cross-lingual capacities of these models, and to provide an equitable information ecosystem accessible to all.

==> src/bak-tab-human_eval_translation_quality.tex <==
\begin{table*}[ht]
\centering
\caption{Metrics for translation quality evaluation}
\label{table:ChatbotTranslationMetrics}
\begin{tabularx}{\textwidth}{l|X}
\hline
\textbf{Category} & \textbf{Description} \\ 
\hline
\multirow{2}{*}{Accurate (1)} & The translation is correct. There are no inaccuracies in terminology translation or the semantic interpretation of the original text.\\
\hline
\multirow{2}{*}{Partially Accurate (0)} & The translation is mostly accurate but contains minor errors, with 1-3 words incorrectly translated. However, these inaccuracies do not significantly distort the overall semantic integrity of the translated text.\\
\hline
\multirow{2}{*}{Inaccurate (-1)} & The translation is substantially flawed with >3 words incorrectly translated or a fundamental distortion of the original text's semantic meaning. \\ % The translated text does not faithfully represent the source material.
\hline
\end{tabularx}
\end{table*}

==> src/bak-tab-translation.tex <==

\begin{table}[ht]
\caption{Comparison of translation quality among the 3 models. }
\setlength{\tabcolsep}{1.0pt}
\small
\begin{tabular}{l|ccc|ccc}
\toprule
Language   &      & Chinese &      &      & Hindi &      \\ \cline{3-3} \cline{6-6}
Rating    & 1    & 0       & -1   & 1    & 0     & -1   \\ 
\midrule
ChatGPT   & 91\% & 8\%     & 1\%  & 75\% & 19\%  & 6\%  \\
Google & 61\% & 36\%    & 3\%  & 80\% & 3\%   & 17\% \\
Marian  & 27\% & 36\%    & 37\% & 12\% & 64\%  & 24\% \\ 
\bottomrule
\end{tabular}
\label{tab:translation}
\end{table}


==> src/fig-consistency_boxplot.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.96\textwidth]{fig/consistency_boxplot.pdf}
    \caption{Comparison of % Sentence embedding similarities
    $\operatorname{sim}_{\text{sent}}$, BERTScore, $\operatorname{sim}_{\text{HDP}}$, and $\operatorname{sim}_{\text{2-gram}}$ on the LiveQA dataset across 5 temperatures ($\tau$) and 4 languages.}
    \label{fig:BERTScore}
%    \vspace{-0.5cm}
\end{figure*}

==> src/fig-verifiability-gpt4.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{fig/verifiabilityGPT4.pdf}
    \caption{Results of GPT-4 in the verifiability experiments on the HealthQA dataset. GPT-4 exhibits better performance compared with GPT-3.5 (Table~\ref{fig:VerifiabilityGPT4}) }
    % \yq{Create bounding box to separate subplots from the main one}
    \label{fig:VerifiabilityGPT4}
    % \vspace{-0.5cm}
\end{figure*}

==> src/fig-verifiability.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.98\textwidth]{fig/verifiability.pdf}
    \caption{Results of HealthQA, LiveQA, and MedicationQA on metrics of the verifiability experiment, including macro precision, macro recall, macro F1-score, accuracy, and area under the curve (AUC). Each column represents a distinct metric. The x- and y-axis of each heatmap represent varying languages and temperatures $\tau$, respectively. 
    \label{fig:VerifiabilityGPT35}
    % \yb{We may use language code (e.g., EN, ES) across the paper? Heatmaps are typically used to represent correlations or relationships between variables. I personally think Figure 3 is more straightforward.}
    % \yb{Minor suggestion: Similar to the comments for Figure 2, if multiple datasets or metrics exhibit the same trend, you may consider displaying only a subset of them to conserve space. For instance, you could choose to showcase F1, accuracy, and AUC, as these are the metrics you discuss in your analysis. }
}
    % \yq{Create bounding box to separate subplots from the main one}
    % \vspace{-0.5cm}
\end{figure*}


==> src/tab-ANOVA_healthqa.tex <==
\begin{table*}
    \centering
    \begin{tabular}{cc|ccccccc}
    \toprule
        $\tau$ & Metric  & $\mathrm{sim}_{\text{sent}}$ & BERTScore & $\operatorname{sim}_{\text{1-gram}}$ & $\operatorname{sim}_{\text{2-gram}}$  & length & $\operatorname{sim}_{\text{LDA}20}$ & $\operatorname{sim}_{\text{HDP}}$ \\ \midrule
        \multirow{2}{*}{0.0} & $\mathcal{F}$ & 153.47 & 157.28 & 190.94 & 201.70 & 35.04 & 47.08 & 33.13  \\ 
          & $p$ & 2.52e-80 & 5.93e-82 & 8.29e-96 & 4.85e-100 & 2.01e-21 & 2.87e-28 & 2.56e-20  \\ \hline
        \multirow{2}{*}{0.25} & $\mathcal{F}$ & 166.37 & 160.62 & 199.13 & 195.95 & 26.95 & 82.49 & 15.83  \\ 
          & $p$ & 7.20e-86 & 1.92e-83 & 3.91e-99 & 6.99e-98 & 1.06e-16 & 3.57e-47 & 4.87e-10  \\ \hline
        \multirow{2}{*}{0.5} & $\mathcal{F}$ & 169.11 & 199.40 & 252.44 & 253.87 & 66.61 & 109.25 & 72.64  \\ 
          & $p$ & 7.35e-87 & 4.79e-99 & 1.04e-118 & 3.27e-119 & 6.90e-39 & 2.77e-60 & 4.68e-42  \\ \hline
        \multirow{2}{*}{0.75} & $\mathcal{F}$ & 36.62 & 41.68 & 64.89 & 76.60 & 12.06 & 31.86 & 7.67  \\ 
          & $p$ & 2.76e-17 & 5.11e-19 & 7.59e-26 & 9.26e-29 & 5.00e-07 & 1.48e-15 & 9.14e-05  \\ \hline
        \multirow{2}{*}{1.0} & $\mathcal{F}$ & 149.11 & 304.02 & 368.81 & 329.65 & 20.21 & 178.26 & 22.48  \\ 
          & $p$ & 3.75e-79 & 3.08e-138 & 1.12e-158 & 1.44e-146 & 1.06e-12 & 1.22e-91 & 4.55e-14 \\
        \bottomrule
    \end{tabular}
    \caption{The $\mathcal{F}$-statistics and the $p$-values of ANOVA on the LiveQA dataset. For all metrics, ANOVA shows statistically significant differences between the mean performances on each metrics}
    \label{tab:ANOVA}
\end{table*}



==> src/tab-consistency_gpt4.tex <==
\begin{table*}
    \centering
    \caption{Results of GPT-4 on the HealthQA dataset.}
    \label{tab:ConsistencyGPT4}
    \begin{tabular}{l|cccccc}
    \toprule
        Language & $\operatorname{sim}_{\text{BERT}}$ & $\operatorname{BERTScore}$ & $\operatorname{sim}_{\text{1gram}}$ & $\operatorname{sim}_{\text{2gram}}$ & Length & $\operatorname{sim}_{\text{HDP}}$ \\ 
        \midrule
        English & 0.9980 $\pm$ 0.0025 & 0.9777 $\pm$ 0.0241 & 0.9167 $\pm$ 0.0864 & 0.8761 $\pm$ 0.1233 & 257.0083 $\pm$ 73.4086 & 0.9958 $\pm$ 0.0153   \\
        Spanish & 0.9973 $\pm$  0.0034 & 0.9759 $\pm$ 0.0256 & 0.9097 $\pm$ 0.0899 & 0.8688 $\pm$ 0.1249 & 197.1868 $\pm$ 54.9768 & 0.9914 $\pm$ 0.0292 \\
        \midrule 
        Language & $\operatorname{sim}_{\text{LDA}}^{10}$ & $\operatorname{sim}_{\text{LDA}}^{20}$ & $\operatorname{sim}_{\text{LDA}}^{50}$ & $\operatorname{sim}_{\text{LDA}}^{100}$ & $\operatorname{sim}_{\text{LDA}}^{200}$ & $\operatorname{sim}_{\text{LDA}}^{500}$ \\
        \midrule
        English & 0.9946 $\pm$ 0.0159 & 0.9932 $\pm$ 0.0173 & 0.9907 $\pm$ 0.0215 & 0.9894 $\pm$ 0.0220 & 0.9895 $\pm$ 0.0468 & 0.9880 $\pm$ 0.0506 \\
        Spanish & 0.9956 $\pm$ 0.0099 & 0.9944 $\pm$ 0.0122 & 0.9934 $\pm$ 0.0187 & 0.9921 $\pm$ 0.0172 & 0.9880 $\pm$ 0.0296 & 0.9880 $\pm$ 0.0339 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> src/tab-metric-descriptions.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{l|l}
        \toprule
        Metric & Description \\ 
        \midrule
        Accuracy & The model should generate factually correct answers. \\ 
        Consistency & The model should generate consistent answers to the same question.  \\ 
        Verifiability & The model should be able to % verify correct claims and distinguish them from the incorrect ones. 
        judge correct claims and to distinguish between what is right and wrong. \\ 
        \bottomrule
    \end{tabular}
    \label{tab:principles}
    \caption{Principles of large language models (LLMs) for answering health queries. }
\end{table*}

==> src/tab-notation.tex <==
\begin{table}[!h]
\small
\centering
\caption{Notations used in this paper.}
\label{tab:notation}
\begin{tabular}{c|l}
\toprule
\textbf{Notation} & \textbf{Description} \\
\midrule
$w_i, \textbf{w}_i$ & a token and its contextualized embedding \\
$q_{\text{E}}, q_{\text{NE}}$ & A question in English / non-English languages \\
$a_{\text{E}}, a_{\text{NE}}$ & An answer in English / non-English languages \\
$s_i$ & a response generated by LLM\\
$D$, $|D|$ & A dataset and the number of examples it contains. \\ 
$|s_i|$ & Number of words in the response $s_i$ \\
$l$ & a language\\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}

==> src/tab-unpaired_t_test.tex <==
\begin{table*}
    \centering
    \small
    \caption{Unpaired t-test results on English (en), Spanish (es), Chinese (zh), and Hindi (hi) on the LiveQA dataset with $\tau=0.0$ and $1.0$. $t$ and $p$ stands for the $t$-statistic and $p$-value, respectively. Asterisks (*) denotes the significance level. `*' indicates p<0.05. `**' indicates p<0.01. `***' indicates p<0.001. % \yb{Regarding denoting significance, underling (Table 5) or using color highlights would look more appealing compared to using crosses and marks for each number (Table 3 and 4) } \gaurav{agree with Yibo. The table can be simplified by using asterisks for denoting different levels of significance and including information about what the asterisks mean in the caption}
    } 
    \label{tab:UnpairedTTest}
    \begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
    \toprule
        \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c|} {$\operatorname{sim}_{\text{BERT}}$}  & \multicolumn{2}{c|}{BERTScore}  & \multicolumn{2}{c|} {$\operatorname{sim}_{\text{1gram}}$}  & \multicolumn{2}{c|}{$\operatorname{sim}_{\text{2grams}}$}  & \multicolumn{2}{c|}{$\operatorname{sim}_{\text{LDA}}^{20}$}  & \multicolumn{2}{c}{$\operatorname{sim}_{\text{HDP}}$}    \\ 
        \midrule
        \multicolumn{2}{c|}{Language} & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$  \\ 
        \midrule
        en & es & 0.83 & 4.07e-01 & 0.79 & 4.30e-01  & 0.83 & 4.04e-01  & 1.04 & 2.97e-01 & 0.63 & 5.27e-01  & 2.66 & 8.13e-03** \\ 
        en & zh & 7.62 & 1.47e-13*** & 8.54 & 2.07e-16*** & 9.27 & 7.98e-19*** & 9.57 & 7.43e-20*** & 4.47 & 1.00e-05*** & 5.90 & 7.13e-09*** \\ 
        en & hi & 16.19 & 8.86e-47*** & 18.75 & 2.22e-58*** & 21.31 & 3.34e-70*** & 22.37 & 4.67e-75*** & 9.47 & 1.63e-19*** & 9.07 & 3.85e-18*** \\ 
        es & zh & 7.10 & 4.92e-12*** & 7.81 & 3.98e-14*** & 8.53 & 2.24e-16*** & 8.71 & 5.88e-17*** & 3.75 & 1.98e-04*** & 3.52 & 4.71e-04***  \\ 
        es & hi & 15.87 & 2.41e-45*** & 18.03 & 4.33e-55*** & 20.62 & 5.64e-67*** & 21.67 & 7.93e-72*** & 8.79 & 3.13e-17*** & 6.77 & 4.13e-11*** \\ 
        zh & hi & 9.96 & 2.93e-21*** & 9.70 & 2.49e-20*** & 11.00 & 4.29e-25*** & 11.42 & 1.03e-26*** & 5.33 & 1.55e-07*** & 3.19 & 1.51e-03** \\ 
        \midrule
        \multicolumn{2}{c|}{$\tau=1.0$} & \multicolumn{2}{c|} {$\operatorname{sim}_{\text{BERT}}$}  & \multicolumn{2}{c|}{BERTScore}  & \multicolumn{2}{c|} {$\operatorname{sim}_{\text{1gram}}$}  & \multicolumn{2}{c|}{$\operatorname{sim}_{\text{2grams}}$}  & \multicolumn{2}{c|}{$\operatorname{sim}_{\text{LDA}}^{20}$}  & \multicolumn{2}{c}{$\operatorname{sim}_{\text{HDP}}$}    \\
        \midrule
          \multicolumn{2}{c|}{Language} & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$ & $t$ & $p$  \\ 
        \midrule
        en & es & 4.58 & 6.03e-06*** & 5.40 & 1.04e-07*** & 5.86 & 8.86e-09*** & 5.93 & 5.93e-09*** & 1.33 & 1.84e-01 & 0.03 & 9.76e-01 \\ 
        en & zh & 7.37 & 7.40e-13*** & 9.96 & 2.37e-21*** & 14.22 & 1.78e-38*** & 12.81 & 1.75e-32*** & 7.21 & 2.28e-12*** & 3.77 & 1.85e-04*** \\ 
        en & hi & 18.02 & 1.13e-55*** & 28.94 & 8.01e-107*** & 31.23 & 4.16e-117*** & 28.71 & 8.70e-106*** & 18.87 & 1.24e-59*** & 6.96 & 1.11e-11*** \\ 
        es & zh & 3.85 & 1.36e-04*** & 5.42 & 9.54e-08*** & 9.53 & 8.49e-20*** & 8.27 & 1.38e-15*** & 6.20 & 1.24e-09*** & 3.92 & 1.00e-04*** \\ 
        es & hi & 15.54 & 2.58e-44*** & 25.30 & 5.03e-90*** & 28.54 & 5.52e-105*** & 28.49 & 8.68e-105*** & 18.10 & 4.75e-56*** & 7.33 & 1.03e-12*** \\ 
        zh & hi & 10.93 & 6.06e-25*** & 17.06 & 3.07e-51*** & 16.72 & 1.12e-49*** & 19.27 & 1.58e-61*** & 11.54 & 2.65e-27*** & 2.82 & 4.95e-03** \\ 
        \bottomrule
    \end{tabular}
\end{table*}

==> src/tab-verifiability_medalpaca.tex <==
\begin{table*}[h]
    \centering
    \caption{Results of verifiability experiments on MedAlpaca-30b.}
    \label{tab:verifiabilityMedalpaca}
    \begin{tabular}{l|ccccc}
    \toprule
        ~ & macro\_precision & macro\_recall & macro\_f1 & accuracy & auc  \\
        \midrule
        en & 0.4538 $\pm$ 0.0793 & 0.4998 $\pm$ 0.0097 & 0.4717 $\pm$ 0.0445 & 0.7638 $\pm$ 0.0322 & 0.4998 $\pm$ 0.0097  \\ 
        es & 0.4983 $\pm$ 0.0423 & 0.4999 $\pm$ 0.0192 & 0.4844 $\pm$ 0.0293 & 0.7524 $\pm$ 0.0270 & 0.4999 $\pm$ 0.0192  \\ 
        zh & 0.5080 $\pm$ 0.0162 & 0.5033 $\pm$ 0.0116 & 0.4677 $\pm$ 0.0535 & 0.5964 $\pm$ 0.2033 & 0.5033 $\pm$ 0.0116  \\ 
        hi & 0.4878 $\pm$ 0.1937 & 0.4953 $\pm$ 0.0271 & 0.4429 $\pm$ 0.0550 & 0.7381 $\pm$ 0.0851 & 0.4953 $\pm$ 0.0271 \\ 
        \bottomrule
    \end{tabular}
\end{table*}
